On the Generalization Power of the Overfitted Three-Layer Neural Tangent Kernel Model

In this paper, we study the generalization performance of overparameterized 3-layer NTK models. We show that, for a specific set of ground-truth functions (which we refer to as the "learnable set"), the test error of the overfitted 3-layer NTK is upper bounded by an expression that decreases with the number of neurons of the two hidden layers. Different from 2-layer NTK where there exists only one hidden-layer, the 3-layer NTK involves interactions between two hidden-layers. Our upper bound reveals that, between the two hidden-layers, the test error descends faster with respect to the number of neurons in the second hidden-layer (the one closer to the output) than with respect to that in the first hidden-layer (the one closer to the input). We also show that the learnable set of 3-layer NTK without bias is no smaller than that of 2-layer NTK models with various choices of bias in the neurons. However, in terms of the actual generalization performance, our results suggest that 3-layer NTK is much less sensitive to the choices of bias than 2-layer NTK, especially when the input dimension is large.

==> proofOnePointFive.tex <==
\section{Proof of Proposition~\ref{prop.boundary_condition}}\label{app.proof_one_point_five}
\begin{proof}
{\color{cyan}
Consider a ground-truth function $f(\xsmall)=\sum_{k=0}^\infty u_k (\xsmall^T \bm{e}_d)^k$ where $u_k\geq 0$ for all $k$. 
Notice that by Lemma~\ref{le.Q_positive}, $(\xsmall^T \bm{e}_d)^k = \sum_{l=0}^i Q(k,l) \Xi_{\bm{0}}^l(\xsmall)$. Thus, we have
\begin{align}\label{eq.temp_012501}
    g=\sum_{l=0}^\infty  \frac{\sum_{k=l}^\infty u_k\cdot Q(k,l)}{\Lambda \cdot c_{\hftb}(l,\bm{0})}\Xi_{\bm{0}}^l(\xsmall).
\end{align}
Therefore, the norm of $g$ is determined by the order of $u_k$ for large $k$.

Consider the following ground-truth function
\begin{align*}
    \fg=\int_{\sd}\KTwo(\frac{d}{d+1}\xsmall^T\bm{z}+\frac{1}{d+1})\delta_{\bm{e}_d}(\bm{z})d\xdensity(\bm{z})=\KTwo(\frac{d}{d+1}\xsmall^T\bm{e}_d+\frac{1}{d+1}).
\end{align*}
We can see that $g=\delta_{\bm{e}_1}$ for $\fg$. 
% We now examine the magnitude of the Taylor coefficients of $\int_{\sd}\KTwo(\frac{d}{d+1}\xsmall^T\bm{z}+\frac{1}{d+1})\delta_{\bm{e}_1}(\bm{z})d\xdensity(\bm{z})$, which equals to $\KTwo(\frac{d}{d+1}\xsmall^T\bm{e}_1+\frac{1}{d+1})$. 
We now examine the order of $u_k$ for $\fg$.
To that end, notice that
\begin{align*}
    \frac{(2k)!}{(k!)^2}\frac{4}{2k+1}\left(\frac{1}{2}\right)^{2k+2}=& \frac{(2k-1)!!}{(2k+1)(2k)!!}.
\end{align*}
By Lemma~\ref{le.wallis_inequality}, we thus have
\begin{align}\label{eq.temp_112801}
    \frac{(2k)!}{(k!)^2}\frac{4}{2k+1}\left(\frac{1}{2}\right)^{2k+2}=\Theta\left(\frac{1}{k^{1.5}}\right).
\end{align}
By Lemma~\ref{le.\taylorCoeff_a_over_\taylorCoeff_0} and Lemma~\ref{le.taylor_of_kernel}, we thus have $u_k=\Theta(k^{-1.5})$. 
By the definition of $\delta$-function, we have $\|g\|_1<\infty$ and $\|g\|_{\infty}=\infty$. Note that $\int_{\sd}\delta_{\bm{e}_1}(\bm{z})\Xi_{\bm{0}}^l(\bm{z}) d\xdensity(\bm{z})=\Xi_{\bm{0}}^l(\bm{e}_d)$. Thus, we have $g(\xsmall)=\sum_{l=0}^\infty \Xi_{\bm{0}}^l(\bm{e}_d)\cdot \Xi_{\bm{0}}^l(\xsmall)$. Comparing it with Eq.~\eqref{eq.temp_012501}, we know that $\|g_{\alpha}\|_\infty < \infty$ if and only if $\alpha < -1.5$ (since for $f_{\infty,\alpha}(\xsmall)$, we have $u_k=\Theta(k^{\alpha})$).
The result of this proposition thus follows.
}
\end{proof}


